Finding extremal periodic orbits with polynomial optimisation, with application to a nine-mode model of shear flow

Tobasco et al. [Physics Letters A, 382:382-386, 2018; see https://doi.org/10.1016/j.physleta.2017.12.023] recently suggested that trajectories of ODE systems that optimize the infinite-time average of a certain observable can be localized using sublevel sets of a function that arise when bounding such averages using so-called auxiliary functions. In this paper we demonstrate that this idea is viable and allows for the computation of extremal unstable periodic orbits (UPOs) for polynomial ODE systems. First, we prove that polynomial optimization is guaranteed to produce auxiliary functions that yield near-sharp bounds on time averages, which is required in order to localize the extremal orbit accurately. Second, we show that points inside the relevant sublevel sets can be computed efficiently through direct nonlinear optimization. Such points provide good initial conditions for UPO computations. As a proof of concept, we then combine these methods with a single-shooting Newton-Raphson algorithm to study extremal UPOs for a nine-dimensional model of sinusoidally forced shear flow. We discover three previously unknown families of UPOs, one of which simultaneously minimizes the mean energy dissipation rate and maximizes the mean perturbation energy relative to the laminar state for Reynolds numbers approximately between 81.24 and 125.

==> SIADS-macros-v3.tex <==
% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{tikz}
\usepackage{bm}
\usepackage{mathtools}	% adjust limits for inf sup
\usepackage{hyperref}
\usepackage{xcolor}

% Avoid widows/orphans
\widowpenalty10000
\clubpenalty10000

% Commands
\newcommand{\R}{\mathbb{R}}				% The reals
\renewcommand{\vec}[1]{\mathbf{#1}} 	% Bold vectors
\newcommand{\Rey}{\mbox{\it Re}} 		% Reynolds number
\newcommand{\given}{\,\vert\,}			% vertical bars with space: "given"
\newcommand{\dt}{\,{\rm d}t} 			% dt
\newcommand{\ssep}{\,;}
\newcommand{\abs}[1]{\left\vert #1 \right\vert}

% MATLAB colours for captions
\definecolor{matlabblue}{rgb}{0,0,1}
\definecolor{matlabred}{rgb}{1,0,0}
\definecolor{matlabgreen}{rgb}{0,0.5,0}
\definecolor{matlaborange}{rgb}{0.8706,0.4902,0}
\definecolor{matlabmagenta}{rgb}{0.7490,0,0.7490}
\definecolor{matlabgrey}{rgb}{0.65,0.65,0.65}

% Lines for figure captions
\newcommand\solidrule[1][10pt]{\rule[0.5ex]{#1}{1.5pt}}
\newcommand\dashedrule{\mbox{%
		\solidrule[2pt]\hspace{2pt}\solidrule[2pt]\hspace{2pt}\solidrule[2pt]}}
\newcommand\dotdashedrule{\mbox{%
		\solidrule[3pt]\hspace{1.5pt}\solidrule[1pt]\hspace{1.5pt}\solidrule[3pt]}}
\newcommand\dottedrule{\mbox{%
		\solidrule[1pt]\hspace{1pt}\solidrule[1pt]\hspace{1pt}\solidrule[1pt]\hspace{1pt}\solidrule[1pt]\hspace{1pt}\solidrule[1pt]\hspace{1pt}}}

% Symbols for figure captions
\newcommand{\mysquare}[1]{%
	\protect\begin{tikzpicture}%
	\protect\draw[thick,color=#1] (0,0) -- (0.75ex,0) -- (0.75ex,0.75ex) -- (0,0.75ex) -- (0,0);
	\protect\end{tikzpicture}%
}
\newcommand{\mytriangle}[1]{%
	\protect\begin{tikzpicture}%
	\protect\draw[thick,color=#1] (0,0) -- (1ex,0) -- (0.5ex,0.866ex) -- (0,0);
	\protect\end{tikzpicture}%
}
\newcommand{\myudtriangle}[1]{%
	\protect\begin{tikzpicture}%
	\protect\draw[thick,color=#1] (0,0.866ex) -- (1ex,0.866ex) -- (0.5ex,0ex) -- (0,0.866ex);
	\protect\end{tikzpicture}%
}
\newcommand{\mycross}[1]{%
	\protect\begin{tikzpicture}%
	\protect\draw[thick,color=#1] (0,0) -- (1ex,1ex);
	\protect\draw[thick,color=#1] (0,1ex) -- (1ex,0);
	\protect\end{tikzpicture}%
}
\newcommand{\mycircle}[1]{%
	\protect\begin{tikzpicture}%
	\protect\draw[thick,color=#1] (0.5ex,0.5ex) circle (0.5ex);
	\protect\end{tikzpicture}%
}

% Math operators
\DeclareMathOperator{\supp}{supp} 				% support

% Alignment in substack
\makeatletter
\newcommand{\subalign}[1]{%
	\vcenter{%
		\Let@ \restore@math@cr \default@tag
		\baselineskip\fontdimen10 \scriptfont\tw@
		\advance\baselineskip\fontdimen12 \scriptfont\tw@
		\lineskip\thr@@\fontdimen8 \scriptfont\thr@@
		\lineskiplimit\lineskip
		\ialign{\hfil$\m@th\scriptstyle##$&$\m@th\scriptstyle{}##$\crcr
			#1\crcr
		}%
	}
}
\makeatother

\ifpdf
\DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
\DeclareGraphicsExtensions{.eps}
\fi

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Finding extremal POs with polynomial optimization}{M. V. Lakshmi, G. Fantuzzi, J. D. F.-Caballero, Y. Hwang, S. I. Chernyshenko}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
%\title{Sum-of-squares approach to finding extremal trajectories, with application to a nine-mode model of shear flow\thanks{Submitted to the editors DATE.
\title{Finding extremal periodic orbits with polynomial optimization, with application to a nine-mode model of shear flow\thanks{Revised version submitted to the editors on {\textcolor{red}{31 January 2020}}.
		\funding{During this work, the first author was supported by EPSRC studentship award 2092930 and the second author was supported by an EPSRC Doctoral Prize Fellowship and an Imperial College Research Fellowship.}}}

%Authors: full names plus addresses.
\author{Mayur V. Lakshmi\thanks{Department of Aeronautics, Imperial College London, Exhibition Road, London, SW7 2AZ, UK
		(\email{mayur.lakshmi11@imperial.ac.uk}, \email{giovanni.fantuzzi10@imperial.ac.uk}, \email{y.hwang@imperial.ac.uk}, \email{s.chernyshenko@imperial.ac.uk}).}
	\and Giovanni Fantuzzi\footnotemark[2]
	\and Jes\'{u}s D. Fern\'{a}ndez-Caballero\thanks{Mathematics Institute, Zeeman Building, University of Warwick, Coventry, CV4 7AL, UK (\email{jesus-david.fernandez-caballero@warwick.ac.uk}).}
	\and Yongyun Hwang\footnotemark[2]
	\and Sergei I. Chernyshenko\footnotemark[2]
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}

%% Optional PDF information
%\ifpdf
%\hypersetup{
%	pdftitle={An Example Article},
%	pdfauthor={D. Doe, P. T. Frank, and J. E. Smith}
%}
%\fi

==> SIADS-macros.tex <==
% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{tikz}
\usepackage{bm}
\usepackage{mathtools}	% adjust limits for inf sup
\usepackage{hyperref}
\usepackage{xcolor}

% Avoid widows/orphans
\widowpenalty10000
\clubpenalty10000

% Commands
\newcommand{\R}{\mathbb{R}}				% The reals
\renewcommand{\vec}[1]{\mathbf{#1}} 	% Bold vectors
\newcommand{\Rey}{\mbox{\it Re}} 		% Reynolds number
\newcommand{\given}{\,\vert\,}			% vertical bars with space: "given"
\newcommand{\dt}{\,{\rm d}t} 			% dt
\newcommand{\ssep}{\,;}
\newcommand{\abs}[1]{\left\vert #1 \right\vert}

% MATLAB colours for captions
\definecolor{matlabblue}{rgb}{0,0,1}
\definecolor{matlabred}{rgb}{1,0,0}
\definecolor{matlabgreen}{rgb}{0,0.5,0}
\definecolor{matlaborange}{rgb}{0.8706,0.4902,0}
\definecolor{matlabmagenta}{rgb}{0.7490,0,0.7490}
\definecolor{matlabgrey}{rgb}{0.65,0.65,0.65}

% Lines for figure captions
\newcommand\solidrule[1][10pt]{\rule[0.5ex]{#1}{1.5pt}}
\newcommand\dashedrule{\mbox{%
		\solidrule[2pt]\hspace{2pt}\solidrule[2pt]\hspace{2pt}\solidrule[2pt]}}
\newcommand\dotdashedrule{\mbox{%
		\solidrule[3pt]\hspace{1.5pt}\solidrule[1pt]\hspace{1.5pt}\solidrule[3pt]}}
\newcommand\dottedrule{\mbox{%
		\solidrule[1pt]\hspace{1pt}\solidrule[1pt]\hspace{1pt}\solidrule[1pt]\hspace{1pt}\solidrule[1pt]\hspace{1pt}\solidrule[1pt]\hspace{1pt}}}

% Symbols for figure captions
\newcommand{\mysquare}[1]{%
	\protect\begin{tikzpicture}%
	\protect\draw[thick,color=#1] (0,0) -- (0.75ex,0) -- (0.75ex,0.75ex) -- (0,0.75ex) -- (0,0);
	\protect\end{tikzpicture}%
}
\newcommand{\mytriangle}[1]{%
	\protect\begin{tikzpicture}%
	\protect\draw[thick,color=#1] (0,0) -- (1ex,0) -- (0.5ex,0.866ex) -- (0,0);
	\protect\end{tikzpicture}%
}
\newcommand{\myudtriangle}[1]{%
	\protect\begin{tikzpicture}%
	\protect\draw[thick,color=#1] (0,0.866ex) -- (1ex,0.866ex) -- (0.5ex,0ex) -- (0,0.866ex);
	\protect\end{tikzpicture}%
}
\newcommand{\mycross}[1]{%
	\protect\begin{tikzpicture}%
	\protect\draw[thick,color=#1] (0,0) -- (1ex,1ex);
	\protect\draw[thick,color=#1] (0,1ex) -- (1ex,0);
	\protect\end{tikzpicture}%
}
\newcommand{\mycircle}[1]{%
	\protect\begin{tikzpicture}%
	\protect\draw[thick,color=#1] (0.5ex,0.5ex) circle (0.5ex);
	\protect\end{tikzpicture}%
}

% Math operators
\DeclareMathOperator{\supp}{supp} 				% support

% Alignment in substack
\makeatletter
\newcommand{\subalign}[1]{%
	\vcenter{%
		\Let@ \restore@math@cr \default@tag
		\baselineskip\fontdimen10 \scriptfont\tw@
		\advance\baselineskip\fontdimen12 \scriptfont\tw@
		\lineskip\thr@@\fontdimen8 \scriptfont\thr@@
		\lineskiplimit\lineskip
		\ialign{\hfil$\m@th\scriptstyle##$&$\m@th\scriptstyle{}##$\crcr
			#1\crcr
		}%
	}
}
\makeatother

\ifpdf
\DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
\DeclareGraphicsExtensions{.eps}
\fi

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Finding extremal POs with polynomial optimization}{M. V. Lakshmi, G. Fantuzzi, J. D. F.-Caballero, Y. Hwang, S. I. Chernyshenko}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
%\title{Sum-of-squares approach to finding extremal trajectories, with application to a nine-mode model of shear flow\thanks{Submitted to the editors DATE.
\title{Finding extremal periodic orbits with polynomial optimization, with application to a nine-mode model of shear flow\thanks{Submitted to the editors June 10, 2019.
		\funding{During this work, the first author was supported by EPSRC studentship award 2092930 and the second author was supported by an EPSRC Doctoral Prize Fellowship and an Imperial College Research Fellowship.}}}

%Authors: full names plus addresses.
\author{Mayur V. Lakshmi\thanks{Department of Aeronautics, Imperial College London, Exhibition Road, London, SW7 2AZ, UK
		(\email{mayur.lakshmi11@imperial.ac.uk}, \email{giovanni.fantuzzi10@imperial.ac.uk}, \email{y.hwang@imperial.ac.uk}, \email{s.chernyshenko@imperial.ac.uk}).}
	\and Giovanni Fantuzzi\footnotemark[2]
	\and Jes\'{u}s D. Fern\'{a}ndez-Caballero\thanks{Mathematics Institute, Zeeman Building, University of Warwick, Coventry, CV4 7AL, UK (\email{jesus-david.fernandez-caballero@warwick.ac.uk}).}
	\and Yongyun Hwang\footnotemark[2]
	\and Sergei I. Chernyshenko\footnotemark[2]
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}

%% Optional PDF information
%\ifpdf
%\hypersetup{
%	pdftitle={An Example Article},
%	pdfauthor={D. Doe, P. T. Frank, and J. E. Smith}
%}
%\fi
